Temporal Context Matters: Enhancing Single Image Prediction with Disease Progression Representations

Clinical outcome or severity prediction from medical images has largely focused on learning representations from single-timepoint or snapshot scans. It has been shown that disease progression can be better characterized by temporal imaging. We therefore hypothesized that outcome predictions can be improved by utilizing the disease progression information from sequential images. We present a deep learning approach that leverages temporal progression information to improve clinical outcome predictions from single-timepoint images. In our method, a self-attention based Temporal Convolutional Network (TCN) is used to learn a representation that is most reflective of the disease trajectory. Meanwhile, a Vision Transformer is pretrained in a self-supervised fashion to extract features from single-timepoint images. The key contribution is to design a recalibration module that employs maximum mean discrepancy loss (MMD) to align distributions of the above two contextual representations. We train our system to predict clinical outcomes and severity grades from single-timepoint images. Experiments on chest and osteoarthritis radiography datasets demonstrate that our approach outperforms other state-of-the-art techniques.

==> method-backup1115-4pm.tex <==
\section{Methodology}
\label{sec:method}

Given a snapshot image of an individual patient, we predict their clinical outcomes/disease severity by utilizing the disease progression information previously learnt from a small temporal dataset with sequential scans. A brief overview of our proposed framework is shown in \cref{overview}. 
The key idea is to use the feature representations of the temporal images to recalibrate the representations of snapshot images. At training stage, besides learning the snapshot representations through the standard loss (e.g., cross-entropy loss or ordinal loss, depending on the tasks), we also match them with the temporal representations at a distribution level, using the MMD loss. At the inference time, the recalibrated snapshot representations are used for the final prediction. 

We use state-of-the-art methods for both the snapshots and the temporal representations. 
This recalibration strategy is elaborated in section \ref{ssec:method2}.
% MMD loss is proposed to recalibrate the snapshot representations according to the most informative feature representation obtained in pretraining phase.  
% %The end-to-end architecture broadly comprises three stages. 
% %In the first stage,
Prior to this, we have two pretraining stages. First, we extract hidden representations from available temporal images of a patient using a hierarchical TCN. This step selects the best representation from each sequence. Detailed description is provided in section \ref{ssec:method1}. Next, a self-supervised vision transformer is trained to extract representations from a large cohort of snapshot images, which has been discussed in section \ref{ssec:method3}. 
%Finally during the downstream evaluation stage,   

%-------------------------------------------------------------------------
\subsection{Temporal Progression Learning}
\label{ssec:method1}
\noindent\textbf{Background:TCN.} The goal of the TCN is to gather the spatial dependencies over long ranges through causal dilated convolutions. Causal nature ensures that the computation of output at an individual timepoint $t$ %takes into account information from % 
depends only on the present and past timepoints. Here, we briefly explain the temporal modeling using a TCN module. 

Assume a sequence of temporal images $\{x_{1}, x_{2},...,x_{T}\}$ available for each patient in the pretraining stage. 
%The images are further divided into a number of grids depending upon the dataset. The grids from the same corresponding parts of each temporal image form a sequence $p=\{p_{1}, p_{2},...,p_{T}\}$. 
These sequence of images are fed to a ResNet-18 model.
% Features are extracted before the fully connected layer.
A vector with 512 elements was obtained with the extracted features. Considering $T$ temporal images of a patient, a sequence of 512-element vectors $p=\{p_{1}, p_{2},...,p_{T}\}$ was computed, which was then used as input to the TCN. 

\cref{architecture} shows the typical structure of a TCN with 2 dilated causal convolution layers. In our architecture we have used 3 such convolution layers. The dilation factors used for the layers are $df = \{1, 2, 4\}$ and the kernel size chosen is $ks = 3$. Dilation is equivalent to introducing a fixed step between every $df$ adjacent filter taps. For a TCN layer, the relevant history information is obtained from $(ks - 1)df$ past timepoints. %A multi-head self attention block is inserted between every two convolutional layers of the TCN. %\cref{attention} shows the structure of one such self-attention block. 
%The TCN operates on the basis of a 1D dilated convolutional layers placed in a hierarchical fashion. 
For an input sequence with $p$ successive images and a filter $f : \{0,..., ks-1\} \rightarrow \mathfrak{R}$, the dilated convolution $D$ on an element $s$ is
defined as:
\begin{equation}
  D(s) = \sum_{j=0}^{ks-1} f(j) \cdot p_{s-df \cdot j} 
  \label{eq:tcn}
\end{equation}
where $s-df\cdot j$ refers to the past direction. 
%Dilation factor $df$ and filter size $ks$ control the working mechanism of TCN. 
%Dilation is equivalent to introducing a fixed step between every $df$ adjacent filter taps. 
%Increasing its value can lead to the increase in depth of the network (i.e., $df = O(2^i)$ at level $j$ of the network). When $df = 1$, a dilated convolution reduces to a regular convolution. Using larger dilation enables an output at the top level to represent a wider range of inputs, thus effectively expanding the receptive field of convolutional layers \cite{method1}. For choosing larger filter sizes $ks$, the effective history of one such layer is $(ks - 1)df$. With above designs, the TCN model is thus able to take similar inputs and produce similar outputs as RNNs while taking advantage of convolution architectures.

\noindent\textbf{Hierarchical attention.}
In addition to feature extraction, we also exploit the TCN structure to zero in on the timepoint which is most optimal representative of the entire image sequence. As shown in \cref{architecture}, a multi-head self attention block is inserted between every two convolutional layers of the TCN. The input features are transformed into query $f$ and key $g$ via $1\times1$ convolutions, The attention map $Att$ is then obtained from $f$ and $g$ by
\begin{equation}
  {Att = \beta(f^{T}g})
  \label{eq:attweight}
\end{equation}

where $\beta$ is the softmax activation function. These maps contain self-attention weights which essentially quantify the importance of one timepoint relative to another. Next, the weighted representations $Att^{T}h$ are generated, where $h$ is another set of feature transformed using $1\times1$ convolution. Finally we add the input features $p$, to $Att^{T}h$. This output representation $o$, as shown in Eqn. \ref{eq:attoutput}, is then used in the recalibration task performed in section \ref{ssec:method2}.

\begin{equation}
  {o = p + Att^{T}h}
  \label{eq:attoutput}
\end{equation}


% The output feature of self-attention block is essentially same as the input obtained from previous convolution layer. However within the block, we collect attention weights from each layer. $W$ is a $T\times T$ self-attention matrix where each row contains the self-attention scores for a particular timepoint. We perform row-wise summation of this attention matrix to obtain an attention vector $Att$. Thus we are able to compute a single attention score for each timepoint. This score is a measure of the correlation shared by an image with its neighboring timepoints. The attention vector of each layer is calculated as:

% \begin{equation}
%   Att_i = \sum_{rows}G_{i}^{T}H_{i} ,     i=1,2,3
%   \label{eq:layeratt}
% \end{equation}

% Eventually the attention scores obtained from 3 layers are added, and a softmax layer is applied to generate the global layered attention vector $G_{Att}$. It is described as:

% \begin{equation}
%   G_{Att} = \sigma(\sum_{i=1}^{3} Att_i)
%   \label{eq:globalatt}
% \end{equation}

% where $\sigma$ is the sigmoid softmax function. Based on the highest attention score in $G_{Att}$, only one representation is selected from each sequence as the optimal representation. This representation is then used in the recalibration task performed in section \ref{ssec:method2}.


%-------------------------------------------------------------------------
\subsection{Recalibration Network}
\label{ssec:method2}
During evaluation on a target dataset, we obtain single timepoint image embeddings $f^{snap}\in\mathbb{R}^{512}$ from the contrastive head in section \ref{ssec:method3}. These are fed as input to a simple neural network with 1 hidden layer. For each snapshot image, we also have optimal representations $f^{temp}\in\mathbb{R}^{512}$ from multiple sequences obtained in section \ref{ssec:method1}. The optimal representations are used only in the training stage. Hence, to train the neural network, we employ modified MMD loss between the features from snapshot and temporal context. MMD loss helps to exploit the underlying disease progression patterns by matching these two representations. The loss in this scenario is calculated by:

\begin{equation}
  \mathcal{L}_{MMD} = argmin\sum_{n=1}^{N}\sum_{k=1}^{TS} \mu (f^{snap}_{n})- \mu (f^{temp}_{k})
  \label{eq:mmd}
\end{equation}
where $N$ is the number of snapshot training samples and $TS$ is the number of temporal sequences.  

\subsection{Snapshot representation learning}
\label{ssec:method3}
We adopt the architecture of Self-supervised image Transformer (SiT) [] without the rotation task. We employ two tokens - first, the image patch token to perform image reconstruction, and second, the contrastive token of SimCLR [] for contrastive prediction task.

\noindent\textbf{Reconstruction task.} We train the transformer as an autoencoder for the visual reconstruction task. The reconstructed image is obtained through the output tokens of the transformer. Transformations are applied to the individual grids of an image. They include addition of random noise, blurring by filters, and random grid replacement from another image. The motivation is to learn domain agnostic representations of relevant organs from the snapshot scans. The transformer aims to restore the original image from the corrupted image. The $\ell1$-loss between the input and the reconstructed image is employed as shown in Equation \ref{eq:recloss}:
\begin{equation}
\label{eq:recloss}
\mathcal{L}_{\rm r}(\mathbf{P}) = \frac{1}{D}\sum_i^D ||I_i - {\rm T}_{\rm r}(\bar{I_i})||
\end{equation}


where, $||.||$ is the $\ell1$ norm, $I_i$ is the original image, $\bar{I_i}$ is the corrupted image, ${\rm T}_{\rm r}(.)$ returns the reconstructed image and $D$ denotes the batch size.  ${P}$ are the parameters of the transformer to be learned during training.

\noindent\textbf{Contrastive learning task.} Simple augmentation techniques like cropping and horizontal flipping are applied on the training samples. Positive pair is constructed with the augmented versions of same image and negative pair denotes samples coming from different inputs. The network is trained with the objective to minimize distance between positive pair and maximize distance between negative pair. This is achieved through a contrastive loss function with cosine similarity as the similarity measure.
\begin{equation}
\label{eq:contrastive}
\mathcal{L}_{\rm c}(\mathbf{P}) = -\frac{1}{D}\sum_{i=1}^D \log \frac{{\rm e}^{{\rm sim}({\rm T}_{\rm c}(I_i), ~{\rm T}_{\rm c}({\tilde I_j}))/\tau}}{\sum_{j=1, j\neq i}^{2D} {\rm e}^{{\rm sim}({\rm T}_{\rm c}(I_i),~{\rm T}_{\rm c}(I_j))/\tau}}
\end{equation}
where ${\rm T}_{\rm c}(.)$ denotes the image embedding coming from the contrastive head, $\rm sim(.,.)$ is the dot product of the $\ell_2$ normalised inputs, which is the cosine similarity, and $\tau$ denotes a constant temperature parameter which we set to $0.5$. ${\tilde I_j}$ is a sample matching in content the sample, $I_j$. The contrastive loss is defined as the arithmetic mean over all positive pairs in the batch of the cross entropy of their normalised similarities.

\subsection{Loss function}
\label{ssec:method4}
For pretraining of snapshot images as discussed in section \ref{ssec:method3}, we used a weighted combination of Reconstruction loss and Contrastive loss. It is given by:

\begin{equation}
  \mathcal{L}_{pre} = \lambda_{p1}\mathcal{L}_{r} +  \lambda_{p2}\mathcal{L}_{c}
  \label{eq:preloss}
\end{equation}

The pretraining of sequential images using TCN is performed with categorical cross entropy loss.

The final loss for finetuning task is different for two types of target datasets. For outcome prediction on chest radiographs, we preferred a combination of proposed MMD loss and Cross-entropy loss \ref{eq:final1}. On the other hand, the severity changes in knee osteoarthritis disease is a classic example of ordinal regression. Hence being inspired by previous works \cite{ordinal}, we used a combination of MMD loss and Ordinal loss \ref{eq:final2}.

\begin{equation}
  \mathcal{L}_{chest} = \lambda_{1}\mathcal{L}_{MMD} + \mathcal{L}_{CE}
  \label{eq:final1}
\end{equation}

\begin{equation}
  \mathcal{L}_{knee} = \lambda_{2}\mathcal{L}_{MMD} + \mathcal{L}_{Ord}
  \label{eq:final2}
\end{equation}


